Constraints on the Physical Properties of GW190814 through Simulations based on DECam Follow-up Observations by the Dark Energy Survey

On 14 August 2019, the LIGO and Virgo Collaborations detected gravitational waves from a black hole and a 2.6 solar mass compact object, possibly the first neutron star -- black hole (NSBH) merger. In search of an optical counterpart, the Dark Energy Survey (DES) obtained deep imaging of the entire 90 percent confidence level localization area with Blanco/DECam 0, 1, 2, 3, 6, and 16 nights after the merger. Objects with varying brightness were detected by the DES Pipeline and we systematically reduced the candidate counterparts through catalog matching, light curve properties, host-galaxy photometric redshifts, SOAR spectroscopic follow-up observations, and machine-learning-based photometric classification. All candidates were rejected as counterparts to the merger. To quantify the sensitivity of our search, we applied our selection criteria to full light curve simulations of supernovae and kilonovae as they would appear in the DECam observations. Since the source class of the merger was uncertain, we utilized an agnostic, three-component kilonova model based on tidally-disrupted NS ejecta properties to quantify our detection efficiency of a counterpart if the merger included a NS. We find that if a kilonova occurred during this merger, configurations where the ejected matter is greater than 0.07 solar masses, has lanthanide abundance less than $10^{-8.56}$, and has a velocity between $0.18c$ and $0.21c$ are disfavored at the $2\sigma$ level. Furthermore, we estimate that our background reduction methods are capable of associating gravitational wave signals with a detected electromagnetic counterpart at the $4\sigma$ level in $95\%$ of future follow-up observations.

==> candidates.tex <==
nqq 624921 20.95506 -33.034762 9
nqr 624609 23.573539 -32.741781 6
noq  624690 12.199493 -25.30652 4 #(panstarrs, 25356, believed AGN at 0.436522)
ntn 624157 23.722289 -31.380485 6 #(growth, 25393)
npw 626761 13.968327 -25.783283 9
num 631360 13.881677 -22.969021 7 #(growth, 25393)
ntr 661833 15.007796 -26.714266 9
omx 625839 24.18436 -33.302678 6
ntp 626956 12.550301, -26.197933 7 #(growth, 25393)
nte 631484 23.557358 -31.7217 1
omw 635566 12.234396 -23.170137 1
